On the Existence of Universal Finite or Pushdown Automata

We investigate the (non)-existence of universal automata for some classes of automata, such as finite automata and pushdown automata, and in particular the influence of the representation and encoding function. An alternative approach, using transition systems, is presented too.

==> eptcsdata.tex <==
\providecommand{\firstpage}{79}
\providecommand{\publicationstatus}{E. Kashefi, J. Krivine, F. van Raamsdonk (Eds.) \\
DCM 2011\\
EPTCS 88, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.88.7}{10.4204/EPTCS.88.7}}

